Extending and Evaluating and Novel Course Reform of introductory Mechanics

The research presented in this thesis was motivated by the need to improve introductory physics courses. Introductory physics courses are generally the first courses in which students learn to create models to solve complex problems. However, many students taking introductory physics courses fail to acquire a command of the concepts, methods and tools presented in these courses. The reforms proposed by this thesis focus on altering the content of introductory courses rather than content delivery methods as most reforms do. This thesis explores how the performance on a widely used test of conceptual understanding in mechanics compares between students taking a course with updated and modified content and students taking a traditional course. Better performance by traditional students was found to stem from their additional practice on the types of items which appeared on the test. The results of this work brought into question the role of the introductory physics course for non-majors. One aspect of this new role is the teaching of new methods such as computation (the use of a computer to solve numerically, simulate and visualize physical problems). This thesis explores the potential benefits for students who learn computation as part of physics course. After students worked through a suite of computational homework problems, many were able to model a new physical situation with which they had no experience. The failure of some students to model this new situation might have stemmed from their unfavorable attitudes towards learning computation. In this thesis, we present the development of a new tool for characterizing students' attitudes. Preliminary measurements indicated significant differences between successful and unsuccessful students.

==> 05-measurement.tex <==
\chapter{Testing Students' Abilities to Solve Mechanics Problems using Computation}
\section{Introduction}
\section{Developing and Deploying a Proctored Computational Instrument}
\section{Challenges to Student Success - A Detailed Analysis of Student Submitted Code}
\section{Implications for Instruction, Laboratory, and Problem Design}


==> caballero-outline.tex <==
\chapter{Introduction}
\section{Reforming Physics Instruction}
\section{Measuring the Effects of Reform}
\section{Research Questions}

\chapter{Background}
\section{Introduction}
\section{Pedagogical Reforms in Introductory Physics}
\section{Research-based Curricular Reform}
\section{Computer Modeling in Introductory Physics}

\chapter{Measurement Techniques}
\section{Introduction}
\section{Quantitiative Data}
\section{Qualitative Data}
\section{Statistical Testing of Significance}
\subsection{Equality of Variance}
\subsection{Equality of Means}
\subsection{Group Effects}
\section{Data Mining Techniques}
\subsection{Principle Component Analysis}
\subsection{Factor Analysis}
\subsection{Cluster Analysis}


\chapter{Curricular Comparison using the Force Concept Inventory}
\section{Introduction}
\section{Mechanics at Georgia Tech}
\section{Summary of Results from In-Class Testing}
\section{Item Analysis of the FCI}
\section{Origins of the Performance Differences}
\section{Discussion of Results}

\chapter{A Novel Application of Cluster Analysis}
\section{Introduction}
\section{Problem Clusters from the Force Concept Inventory}
\section{Response Modes from the Force Concept Inventory}
\section{Discussion of Results}

\chapter{Computation in Introductory Mechanics}
\section{Introduction}
\section{Computational Instruction at Georgia Tech}
\subsection{Mechanics Laboratories}
\subsection{Computational Homework Exercises}
\section{Measuring Student Performance on Computational Exercises}
\subsection{Proctored Computational Assignment}
\subsection{Common Coding Mistakes}
\subsection{Implications for Instruction}
\section{A New Tool for Measuring Attitudes and Beliefs about Computation}
\subsection{Computational Modeling in Physics Attitudinal Student Survey}
\subsection{Measurements of Students' Computational Anxiety}
\section{Discussion of Results}

\chapter{Conclusion and Summary}
\section{Discussion}
\section{Future Research Directions}
\section{Closing Remarks}


==> vpython/background.tex <==
\section{Computational Modeling in Introductory Physics: A short history}\label{sec:history}

Using computational modeling in an introductory physics course is not a new idea. In fact, several notable attempts have been made since the development of small, relatively cheap, modern microcomputers with visual displays in the 1980's. Furthermore, since the early 2000's the ubiquity of fast and reliable internet connectivity has helped propagate computational ideas, scripts, and programming environments among developers, instructors, and students.

%One of the earliest attempts to introduce computational physics to introductory physics students occurred 
In the late 1980's, the Maryland University Project in Physics and Educational Technology (M.U.P.P.E.T.) was relatively successful with a small number of physics majors (many of which had some programming experience). In the M.U.P.P.E.T environment, students developed iterative procedures using Turbo Pascal. 
%It was believed that by learning Pascal, students would obtain skills that were transferrable to professional languages such as C and FORTRAN; languages which students might encounter in their future careers. Pascal requires the explicit declaration of variables and does not automatically generate graphics as more modern languages can. 
Due to the hardware and software limitations at the time, interactive 3D graphics were not possible; output was limited to graphs. 
%The M.U.P.P.E.T. literature describes in detail how it was used in classses and how it altered what material could be covered in an introductory physics course. Less is said about using M.U.P.P.E.T. as an educational tool to develop conceptual understanding or what types of difficulties students encountered using M.U.P.P.E.T. to solve problems. 
Redish and Wilson report that some students in their second and third year of physics study were able to use M.U.P.P.E.T. for independent research projects that were ``valuable and interesting'' \cite{macdonald1988muppet, redish1993student}. 
%These projects also led to increased student interest in continuing independent research later in students' academic careers. 
The use of Turbo Pascal required that students learn the details of a programming language which might have hindered adoption at lower levels. 
%Future efforts would attempt to reduce the cognitive effort devoted to learning syntax and semantics by developing graphical programming environments.

%% Reread STELLA papers

Students who learned to use the graphical modeling package STELLA, developed by Niedderer and colleagues, to model physical systems were not burdened with learning a programming language (like Pascal). STELLA developers desired that students solve more complex problems than simple algebraic solution strategies allowed but believed that learning programming languages placed too much emphasis on symbolic equations and, hence, were too difficult to learn hindering use a lower levels (e.g., high school) \cite{schecker1993learning}. 
%STELLA was a graphical programming environment in which students created links between ``Box'' icons (which represented quantities to be summed or integrated) and ``Flow'' icons (which represented the rate of change of summed quantities). Students could numerically integrate systems by correctly linking ``Flow'' icons to the appropriate ``Box'' icons. 
The barrier for adoption was low enough for STELLA ( compared to M.U.P.P.E.T.) that it could be used in upper level high school physics. Schecker noted that course content changed from ``canned'' closed-form problems to open-ended and inquiry-based projects. In fact, student-student and student-instructor interaction increased as a result of using STELLA \cite{schecker1994system}. 
%%REwrite?
%Furthermore, Schecker found that students' conceptual understanding of certain physical phenomenon was altered by using STELLA; students began to qualitatively assess the physical situtation rather than simply plugging in numbers.

%% Read BOXER papers carefully

More powerful and generalizable than STELLA, BOXER was developed by researchers at the University of California Berkeley as an outgrowth of their successful programming language Logo. BOXER was a flexible programming environment;
% which crossed the line between text-based and graphical programming. While 
users wrote procedures and subroutines line-by-line, but much of BOXER's organization scheme was graphical \cite{disessa1986boxer}. 
%Data structures, subroutines, and graphical output were sectioned off into boxes within the programming environment. The Berkeley group experimented with high school student programming in BOXER to explore concepts in physics. 
High school physics students learned the basics of BOXER programming and explored a wide variety of physical phenomenon using instructor developed programs \cite{sherin1993dynaturtle}. Using collaborative discussion and development, programs were refined, often by instructors, to develop a computational model which represented visually the expected motion \cite{disessa1995designing}. %In diSessa's words, the goal of the project was to have students ``design Newton's Laws'' by using an iterative design procedure .

More modern efforts into the development of computational modeling have had the advantage of cheap and available hardware, fast internet connections, and efficient video cards capable of rendering 3D graphical environments. As a result, many efforts have focused on developing simulations -- computational modeling programs in which the user has little or no access to the underlying model or modeling algorithm. User interaction might be limited to setting or adjusting parameters and mouse or keyboard interactivity. The advantage of simulations is that they are, often, professionally constructed and tested, run similarly on a variety platforms with little more than an internet browser, and can be highly visual. The University of Colorado at Boulder's PhET group has developed a suite of these simulations which cover a wide variety of physical phenomenon for use in all levels of physics and physical science \cite{perkins2006phet,wieman2006powerful}. We distinguish computational modeling from simulation because students are not building the underlying model and do not have access to that model; students interact with simulations but construct computational models. 

Computational modeling efforts have also benefited from the development of high-level, object-oriented programming languages. Computational modeling, as we have defined it, includes the writing of program statements, the creation of objects, and the debugging of errors. Using high-level languages such as C, JAVA, and Python to develop computational models meet this definition. Students who learn one of these programming languages have the advantage of peering into the ``black box'' to view and to alter the underlying algorithm on which the model depends. Furthermore, students can learn to develop their own computer models which solve new and different problems. But, students must devote additional time and cognitive effort to learning syntax and procedures to construct their own models. And depending on the particular environment, students might devote more time and cognitive effort to the details of constructing a working model (e.g., message handling, drawing graphics, garbage collection) than the physics behind the model.

To teach computation in introductory physics, a powerful and flexible 3D modeling environment with a minimal programming barrier is needed. Significant efforts were made by Sherwood and co-workers to develop one such environment for introductory physics. VPython was created to teach computational modeling to physics students at Carnegie Mellon University \cite{computajp}. It contains features that make writing programs to simulate physical systems simple and straight-forward \cite{vpythonWebsite}. VPython is not a ``black-box'' environment; students write all the program statements necessary to model the physical system. The additional details of program construction (e.g., drawing graphics, creating windows, mouse interactions) are handled by VPython; this allows the student to focus on the core details of the model. The VPython programming environment supports full 3D graphics and animation without the additional burden to students of learning object-oriented programming. 
Other attempts have been made to embed computational physics into introductory courses. These curricula utilize pre-constructed simulations or programming environments in which the students' experience is limited to changing initial conditions and selecting features of the solution (i.e., plots, tables, etc.) \cite{christian2007modeling,teodoro2010mathematical,neves2010improving}. By contrast, students are readily developing computational models using Python, JAVA, C, and MATLAB in intermediate and advanced courses.
 

